Feature Alignment with Equivariant Convolutions for Burst Image Super-Resolution

Burst image processing (BIP), which captures and integrates multiple frames into a single high-quality image, is widely used in consumer cameras. As a typical BIP task, Burst Image Super-Resolution (BISR) has achieved notable progress through deep learning in recent years. Existing BISR methods typically involve three key stages: alignment, upsampling, and fusion, often in varying orders and implementations. Among these stages, alignment is particularly critical for ensuring accurate feature matching and further reconstruction. However, existing methods often rely on techniques such as deformable convolutions and optical flow to realize alignment, which either focus only on local transformations or lack theoretical grounding, thereby limiting their performance. To alleviate these issues, we propose a novel framework for BISR, featuring an equivariant convolution-based alignment, ensuring consistent transformations between the image and feature domains. This enables the alignment transformation to be learned via explicit supervision in the image domain and easily applied in the feature domain in a theoretically sound way, effectively improving alignment accuracy. Additionally, we design an effective reconstruction module with advanced deep architectures for upsampling and fusion to obtain the final BISR result. Extensive experiments on BISR benchmarks show the superior performance of our approach in both quantitative metrics and visual quality.

==> 03_method.tex <==


\section{Method}
\label{sec:method}
We propose a Burst Image multi-scale super-resolution method with equivariant convolutions. 
This section first presents the preliminaries of equivariant convolutions to establish the foundational knowledge required to understand the proposed method. Following this, we provide a detailed description of the network architectures and offer a theoretical justification to substantiate the validity and robustness of the proposed approach.

\subsection{Preliminary \label{sec:pre}}
Building on prior works \cite{fconv, fonvunfolding}, the concept of equivariance for a mapping refers to the property where a transformation applied to the input results in a corresponding, predictable transformation on the output. Specifically, let \( g \) denote a mapping from the input feature space to the output feature space, and let \( F \) represent a group of transformations. We say that \( g \) is equivariant with respect to \( F \) if, for any \( f \in F \), the following condition holds:

\begin{equation}
    f^{'}[g[x]] =  g[f[x]],
\end{equation}

where \( x \) is any feature map from the input space, and \( f[\cdot] \) and \( f^{'}[\cdot] \) denote the actions of the transformation \( f \) on the input and output features, respectively.
It is important to note that, in this paper, we focus on rotation and translation equivariance, which are particularly relevant to the specific degradation observed in burst images, within the context of 2D convolutions. In this setting, \( F \) represents the group of rotation and translation transformations, and \( g \) denotes the convolution mapping.



\subsection{Our method}

Given $B$ burst RAW low-resolution (LR) images $\{I_j^{L}\}_{j=0}^{B-1}$, where each image $I_j^{L} \in \mathbb{R}^{1 \times h \times w}$, the raw input images are first processed into a 4-channel format following the 'RGGB' Bayer pattern, as in previous works \cite{kang2025burstm, dudhane2023burstormer}. Among these burst images, one is selected as the base frame, which serves as the reference for high-resolution (HR) reconstruction, while the remaining frames are used to assist in super-resolving the base frame. The proposed network is then employed to upsample the base frame by a factor of $s$, resulting in an HR image in the sRGB format with 3 channels.
We propose a multi-scale burst image super-resolution (BISR) network that aligns with the pipeline of feature extraction and alignment, feature fusion, and upsampling.

\subsubsection{Alignment with equivariant convolutions}

% Alignment is crucial yet challenging, as it directly affects the quality of the reconstructed high-resolution image.
Misalignment between adjacent frames in burst images, captured in rapid succession, is primarily caused by physical motions, which can be effectively modeled as a combination of rotation and translation. 
As discussed in the Introduction, existing methods face certain challenges and limitations. To address these issues, we propose an \textbf{alignment module} with equivariant convolutions, which supports supervised and global alignment and integrates alignment and feature extraction into a unified framework.
% We ensure more reliable alignment by simplifying the complex transformations to these two kinds of affine operations, providing a solid foundation for burst image super-resolution.

Let \( I_0^L \) be the RAW LR base frame and \( \{I_j^L\}_{j=1}^{B-1}\) be other frames in the burst sequence.
The relationship between the base and one of the other misaligned frames can be modeled using an affine transformation \( f \), which represents rotation and translation. Specifically, the frame \( I_j^L\) is obtained by applying \( f_j \) to the base frame \( I_0^L \):

\begin{align}
    I_j^L = f_j(I_0^L).\label{eq:e_i}
\end{align}

After feature extraction via a network \( g \), the features \( x_0 = g(I_0^L) \) and \( x_j = g(I_j^L) \) are obtained. If \( g \) is equivariant to \( f_j \), then:
\begin{align}
    x_j = g[f_j(I_0^L)] = f_j[g(I_0^L)] = f_j(x_0).\label{eq:e_x}
\end{align}
Combining Eq. \eqref{eq:e_i} and Eq. \eqref{eq:e_x}, we observe that \( f_j \) operates consistently in both the image and feature domains, ensuring alignment consistency.
Consequently, the alignment loss can be defined in the image domain as:
\begin{equation}
    Loss_{\text{align}} = \frac{1}{B-1} \sum_{j=1}^{B-1} \| f_j^{-1}(I_j^L) - I_0^L \|_F^2,\label{eq:loss_align}
\end{equation}
and the aligned features \( \{\tilde{x}_j\}_{j=1}^{B-1} \) are then obtained as:
\begin{align}
    \tilde{x}_j = f_j^{-1}(x_j).
\end{align}

In contrast to deformable convolutions, which learn offsets at the pixel level locally, we model the affine transformations \( \{f_j\}_{j=1}^{B-1} \) globally using learnable affine matrices. Specifically, the transformation matrix \( M_{f_j} \in \mathbb{R}^{2 \times 3} \) is computed as:
\begin{equation}
    M_{f_j} = \phi_{f_j}(\text{concat}[x_0,x_j]),
\end{equation}
where \( \phi_{f_j}(\cdot) \) denotes the convolution layers, and \( \text{concat}[\cdot, \cdot] \) refers to the concatenation operation.


Besides the advances discussed above, equivariant convolutions also perform outstandingly in capturing image priors and extracting features, particularly in image super-resolution tasks \cite{xie2022fourier, fonvunfolding}.




\subsubsection{Feature fusion}
Before upsampling, integrating aligned features is essential to enrich the base frame with relevant information while minimizing redundancy. 
Existing methods either concatenate base and auxiliary features directly \cite{bipnet, dudhane2023burstormer, kang2025burstm} or assign pixel-wise fusion weights via attention maps \cite{fbanet}, computed from element-wise products and Euclidean metrics. Nevertheless, more efficient and effective integration approaches are yet to be explored.

Restormer \cite{zamir2022restormer} is a Transformer-based architecture that has demonstrated strong performance in image restoration tasks, whose core module, Multi-Dconv Head Transposed Attention (MDTA), applies self-attention (SA) across channels instead of the spatial dimension. Specifically, it computes cross-covariance across channels to generate an attention map that implicitly encodes global context. This mechanism can be used to integrate aligned features by modeling the dependencies between the base and the auxiliary features. The fusion module for base and $j_{th}, (j=0,\cdots,B-1)$ features as follows:
\begin{align}
\textbf{Q}_j &= W_d^QW_p^Q(\text{concat}[\tilde{x}_j, x_0]), \\
\textbf{K}_j &= W_d^KW_p^K(\text{concat}[\tilde{x}_j, x_0]), \\
\textbf{V}_j &= W_d^VW_p^V(\text{concat}[\tilde{x}_j, x_0]), \\
\hat{x}_j & = \mathbf{V}_j \cdot \text{Softmax}(\mathbf{K}_j \cdot \mathbf{Q}_j/\alpha_j) + \tilde{x}_j,
\end{align}
where $\{\hat{x}_j\}_{j=0}^{B-1}$ are the fused features, $W_p^{(\cdot)}$ and $W_d^{(\cdot)}$ refers to $1\times1$ pixel-wise and $3\times3$ depth-wise convolutions, respectively, and $\alpha$ is learnable scaling parameter. 

The term $\text{Softmax}(\mathbf{K}_j \cdot \mathbf{Q}_j/\alpha)$  captures feature correlations by weighting the value vectors based on their similarity, enabling a more context-aware fusion.
Unlike element-wise multiplication or concatenation, the attention mechanism captures global correlations and explicitly adjusts feature contributions dynamically, ensuring more effective integration through the well-designed module.


\subsubsection{Upsampling with INR}

For upsampling, we adopt the LTE \cite{lte} framework, which combines the strengths of INR and frequency domain processing for high-frequency information reconstruction. This choice is motivated by two key reasons. First, BurstM \cite{kang2025burstm} has proven the effectiveness of the LTE-based architecture in multi-scale burst image super-resolution. Second, grid sampling, a core component of INR, facilitates the upsampling of sub-pixel information extracted from the original frames. This is particularly critical for burst images, where slight camera shifts during capture introduce fine-grained details that can be effectively recovered. Leveraging grid sampling ensures that these details are preserved and enhanced throughout the upsampling process. 
The final output $I^S\in \mathbb{R}^{3\times sh\times sw}$ in sRGB format can be attained by:
\begin{equation}
    I^S = \text{PS}(\tilde{I}_0^L\uparrow+ {Avg}_{W}[\Phi_{up_j}(\hat{x}_j)]),
\end{equation}
where $\text{PS}(\cdot)$ refers to the pixel shuffle operation,$\tilde{I}_0^L\uparrow \in \mathbb{R}^{12 \times (sh/2) \times (sw/2) }$ refers to the upsampled base frame with bilinear interpolation, ${Avg}_{W}(\cdot)$ refers to the average operation with weighting parameters learned with convolutions from $\hat{x}_j\text{s}$, and $\Phi_{up_j}(\cdot)$ refers to the upsampling module based on LTE. The detailed architecture will be depicted in the supplementary material considering the space limitation.

The final loss of the whole network is composed of two parts as follows:
\begin{align}
    &Loss = Loss_{\text{fidelity}} + Loss_{\text{align}},\\
     &Loss_{\text{fidelity}} = ||I^S, I^{\text{GT}}||_1.
\end{align}



\subsection{Discussion}
This section provides a detailed discussion of the proposed alignment module with rotation-translation equivariant convolutions, supported by theoretical insights and error analysis.

\subsubsection{Equivariant convolutions in continuous domain. }
\textbf{Notations.}

\begin{table}
% \small
  \caption{The involved concepts and notations for equivariant convolutions (eConv) in the continuous and discrete domains, respectively.  } \vspace{-2mm}
  \label{Notation-table}
  \centering \setlength{\tabcolsep}{8pt}
  \begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}{Concept}     &\multicolumn{2}{c}{Notation}   \\
    \cmidrule(r){2-3}
             &   Continuous    & Discrete \\
    \midrule
    Input Image & $r(x)$       & $I$             \\
    Rotation Group &      $O(2)$         &  $S$           \\
    Translation Group &      $(\mathbb{R}^2, +)$         &  $L$           \\
    Rotation element/Index&      $A,D \in O(2)$  &  $A,D \in S$                            \\
    Translation element/Index&      $b \in (\mathbb{R}^2, +$  &  $b \in L$                            \\
    Feature Map & $e(x,A,b)$  & $F^A_b$  \\
    \midrule
    Filter (Input) & $ \varphi_{in}\left(A^{-1}x\right) $     &   $\tilde{\Psi}^A$ \\
    Filter (Intermediate) & $ \varphi_{A}\left(D^{-1}x\right) $     &   $\tilde{\Phi}^{D,A}$ \\
    Filter (Output) & $ \varphi_{out}\left(D^{-1}x\right) $     &   $\tilde{\Upsilon}^D$ \\
    \midrule
    eConv (Input) & $\Psi[r]$ &  $\tilde{\Psi} \star I$ \\
    eConv (Intermediate) & $\Phi[e]$ &  $\tilde{\Phi} \star F$ \\
    eConv (Output) & $\Upsilon[e]$ &  $\tilde{\Upsilon} \star F$ \\
    \bottomrule
  \end{tabular}\vspace{-1.5mm}
\end{table}


Specifically, we represent an image as a two-dimensional grid function $I \in\mathbb{R}^{n\times n}$, and represent an intermediate feature map as $F$. Note that in rotation-translation equivariant networks, a feature map is a multi-channel matrix (i.e., a tensor), with $F\in\mathbb{R}^{n\times n\times t\times l}$, where the third mode is with respect to the rotation group $S$, and $t$ is the number of elements in $S$; the fourth mode is with respect to the translation group $L$, and $l$ is the number of elements in $L$. 
Moreover, we denote a specific channel in $F$ as $F^A_b\in\mathbb{R}^{n\times n}$,  where $A\in S$ is a rotation matrix, $b\in L$ is a translation matrix.
% and also used as an index for denoting a specific channel in $F$.

In the continuous domain, we follow the previous works \cite{xie2022fourier, NEURIPS2019_45d6637b}, considering the equivariance on the orthogonal group  $O(2)$\footnote{The rotation group  $S$ represents a subgroup of $O(2)$, and it is also regarded as the discretization of $O(2)$ in this paper.}, and the translation group $(\mathbb{R}^2,+)$\footnote{The translation group  $L$ represents a subgroup of $(\mathbb{R}^2,+)$, and it is also regarded as the discretization of $(\mathbb{R}^2,+)$ in this paper.} . 
Formally,
$O(2)=\{A\in\mathbb{R}^{2\times 2}|A^TA = I_{2\times  2}\}$, which contains all rotation matrices. 
Without ambiguity, we use $A$ to parameterize $O(2)$. We consider the Euclidean group $E(2) \cong (\mathbb{R}^2,+) \rtimes O(2)$ ($\rtimes$ is a semidirect-product), whose element is represented as $(x, A, b)$. Restricting the domain of $A$, $b$ and $x$, we can also use this representation to parameterize any subgroup of $E(2)$.
The input image can be modeled as a function defined on $\mathbb{R}^2$, denoted as $r(x)$. The intermediate feature map can be model as a function defined on $E(2)$, denoted as $e(x,A, b)$ (as shown in Table \ref{Notation-table}, and $r(x)$ and $e(x,A,b)$ are the continuous versions of $I$ and $F^A_b$, respectively).
We denote the function spaces of $r$ and $e$ as $C^\infty(\mathbb{R}^2)$ and $C^\infty(E(2))$,
respectively\footnote{The smoothness of e means that the feature map $e(x,A,b)$ is smooth with respect to $x$ when $A$ is fixed.
For simplicity, we set the functional space as $C^\infty(\mathbb{R}^2)$. Actually,  in implementation, we only require that $r\in C^2(\mathbb{R}^2)$.
The requirement on $e$ is the same.}.
For an input $r\in C^\infty(\mathbb{R}^2)$ and transformations $\tilde{A}\in O(2)$ and $\tilde{b}\in (\mathbb{R}^2,+))$,  $\tilde{A}$ acts on $r$ by
\begin{equation}\label{piR}
  f^R_{\tilde{A}\tilde{b}}[r](x) = r(\tilde{A}^{-1}(x-b)), \forall x\in\mathbb{R}^2.
\end{equation}
For a feature map $e\in C^\infty(E(2))$ and a transformation $\tilde{A}\in O(2)$, $\tilde{A}$ act on $e$ by
\begin{equation}\label{piE}
  f^E_{\tilde{A}\tilde{b}}[e](x,A,b) = e(\tilde{A}^{-1}(x-b),\tilde{A}^{-1}A), \forall (x,A,b)\in E(2).
\end{equation}
 $\Psi$ denotes the convolution on the input layer,
which maps an input $r\in C^\infty(\mathbb{R}^2)$ to a feature map defined on $E(2)$:
\begin{equation}\label{input_Conv}
  \Psi[r](y,A) =  \int_{\mathbb{R}^2}\varphi_{in}\left(A^{-1}x\right)r(y-x)d\sigma(x),
\end{equation}
$\forall (y, A)\in E(2)$, where $\sigma$ is a measure on $\mathbb{R}^2$ and $\varphi$ is the proposed parameterized filter.
 $\Phi$  denotes the convolution on the intermediate layer,
which maps a feature map $e\in C^\infty(E(2))$ to another feature map defined on $E(2)$:
\begin{equation}\label{regular_Conv}
\begin{split}
   \Phi[e](y,\!D) \!\!=\!\!\!
   \int_{\!O(2)}\!\int_{\mathbb{R}^2}\!\!\varphi_{\!A}\!\left(D^{-\!1}x\right)\!e(y\!-\!x, \!D\!A)d\sigma(x)dv(A),
\end{split}
\end{equation}
$ \forall (y, D)\in E(2)$, where $v$ is a measure on $O(2)$, $A,D\in O(2)$ denotes orthogonal transformations in the considered group,
and $\varphi_{\tilde{A}}$ indicates the filter with respect to the channel of feature map indexed by $\tilde{A}$, i.e., $\left.e(x,A,b)\right|_{A = \tilde{A}}$.
 $\Upsilon$  denotes the convolution on final layer,
which maps a feature map $e\in C^\infty(E(2))$ to a function defined on $\mathbb{R}^2$:
\begin{equation}\label{output_Conv}
  \Upsilon[e](y) \!=\!  \int_{O(2)}\int_{\mathbb{R}^2}\!\!\!\varphi_{out}\!\left(D^{-1}x\right)e(y\!-\!x, D)d\sigma(x)dv(D),
\end{equation}
$\forall y\in \mathbb{R}^2$. Then we can prove the following result:

\begin{Rem} For $r\in C^\infty(\mathbb{R}^2)$, $e\in C^\infty(E(2))$ and $\tilde{A}\in O(2)$,
the following results are satisfied:
\begin{equation}\label{Thm2}
\begin{split}
  \Psi\left[f_{\tilde{A}\tilde{b}}^R\left[r\right]\right] &= f^E_{\tilde{A}\tilde{b}}\left[\Psi\left[r\right]\right],\\
  \Phi\left[f_{\tilde{A}\tilde{b}}^E\left[e\right]\right] &= f_{\tilde{A}\tilde{b}}^E\left[\Phi\left[e\right]\right],\\
  \Upsilon\left[f_{\tilde{A}\tilde{b}}^E\left[e\right]\right] &= f_{\tilde{A}\tilde{b}}^R\left[\Upsilon\left[e\right]\right],\\
\end{split}
\end{equation}
where $f_{\tilde{A}\tilde{b}}^R$, $f_{\tilde{A}\tilde{b}}^E$, $\Psi$, $\Phi$ and $\Upsilon$
are defined by (\ref{piR}), (\ref{piE}), (\ref{input_Conv}), (\ref{regular_Conv}) and (\ref{output_Conv}), respectively.
\end{Rem}


\subsubsection{Equivariant convolutions in discrete domain. }
\begin{theorem}

{\color{red}\textbf{Brief Version}}

Let \( g_{eq}(\cdot) \) represent a one-layer rotation and translation equivariant convolution operation with equivariance order \( t \), and let \( f(\cdot) \) denote an affine transformation, including rotation and translation, applied to an input image (or feature map) \( X \). Under suitable smoothness conditions on \( X \) and the convolution filters, the following inequality holds:
\begin{equation}
    \left| f^{-1} \left[ g_{eq} \right] (f(X)) - g_{eq}(X) \right| \leq C (p+1)^2 h^2,\label{eq:th1}
\end{equation}
where \( f^{-1}(\cdot) \) is the inverse transformation of \( f(\cdot) \), \( h \) is the mesh size, \( p \) is the filter size, and \( C \) is a positive constant independent of \( h \) and \( p \).
\end{theorem}

{\color{red}\textbf{Detailed Version}}

\textbf{Notations.}
We assume that an image $I \in R^{n\times n}$ represents a two-dimensional grid function obtained by discretizing a smooth function, i.e., for $i, j = 1,2, \cdots, n$,
\begin{equation}\label{I}
  I_{ij} = r(x_{ij}),
\end{equation}
where $x_{ij} = \left(\left(i-\frac{n+1}{2}\right)h, \left(j-\frac{n+1}{2}\right)h\right)^T$. We represent  $F$ as a three-dimensional grid function sampled from a smooth function $e: \mathbb{R}^2\times S\to \mathbb{R}$, i.e., for $i, j = 1,2, \cdots, n$,
\begin{equation}\label{F}
  F_{ij}^Ab = e(x_{ij}, A, b),
\end{equation}
where $x_{ij} = \left(\left(i-\frac{n+1}{2}\right)h, \left(j-\frac{n+1}{2}\right)h\right)^T$ and $A\in S$, $S$ is a subgroup of $O(2)$, and $b\in L$, $L$ is a subgroup of $(\mathbb{R},+)$. For $i, j = 1,2, \cdots, p$, and $A,D\in S$, we have
\begin{equation}\label{Phi_d}
\begin{split}
  &\tilde{\Psi}_{ij}^A = \varphi_{in}\left(A^{-1}x_{ij}\right),\\
 &\tilde{\Phi}_{ij}^{D,A} = \varphi_A\left(D^{-1}x_{ij}\right),\\
  &\tilde{\Upsilon}_{ij}^{A} = \varphi_{out}\left(A^{-1}x_{ij}\right),
\end{split}
\end{equation}
where $x_{ij} = \left(\left(i-\nicefrac{(p+1)}{2}\right)h, \left(j-\nicefrac{(p+1)}{2}\right)h\right)^T$, and $\varphi$ and $\varphi_A$ are parameterized filters.
Let
\begin{equation}\label{xy}
\begin{split}
    x_{ij} &= \left(\left(i-\frac{p+1}{2}\right)h, \left(j-\frac{p+1}{2}\right)h\right)^T,\\
    y_{ij} &= \left(\left(i-\frac{n+p+2}{2}\right)h, \left(j-\frac{n+p+2}{2}\right)h\right)^T.
\end{split}
\end{equation}
For $\forall A\in S$ and $i,j = 1,2,\cdots,n,$ the convolution of $\tilde{\Psi}$ and $I$ is
\begin{equation}\label{input_d}
\begin{split}
  \left(\tilde{\Psi}\star I\right)^A_{ij} &=  \sum_{(\tilde{i},\tilde{j})\in\Lambda}\varphi_{in}\left(A^{-1}x_{\tilde{i}\tilde{j}}\right)r\left(y_{ij}-x_{\tilde{i},\tilde{j}}\right),\\
\end{split}
\end{equation}
where  $\Lambda$ is a set of indexes, denoted as $ \Lambda = \{(i,j)|i,j=1,2,\cdots,p\}$, and  $*$ represents the common 2D convolution.
For any $D\in S$ and $i,j = 1,2,\cdots,n,$ the convolution of $\tilde{\Phi}$ and $F$ is
\begin{equation}\label{regular_d}
\color{red}
\begin{split}
    \left(\tilde{\Phi}\star F\right)^D_{ij} &=  \!\!\!\sum_{(\tilde{i},\tilde{j})\in\Lambda, A\in S} \!\!\!\! \varphi_{A}\left(D^{-1}x_{\tilde{i}\tilde{j}}\right)e\!\left(y_{ij}, DA, -x_{\tilde{i},\tilde{j}}\right), \\
\end{split}
\end{equation}
where $\Lambda = \{(i,j)|i,j=1,2,\cdots,p\}$.
For $i,j = 1,2,\cdots,n,$ the convolution of $\tilde{\Upsilon}$ and $F$ is
\begin{equation}\label{output_d}
\color{red}
\begin{split}
   \left(\tilde{\Upsilon}\star F\right)_{ij} &=  \!\!\!\sum_{(\tilde{i},\tilde{j})\in\Lambda, D\in S}\!\!\!\!\varphi_{out}\left(D^{-1}x_{\tilde{i}\tilde{j}}\right)e\!\left(y_{ij}, D, -x_{\tilde{i},\tilde{j}} \right)\\
\end{split}
\end{equation}
where $\Lambda = \{(i,j)|i,j=1,2,\cdots,p\}$.

The transformations on $I$ and $F$ are defined by
\begin{equation}\label{Pi_d}
\begin{split}
    & \left(\tilde{f}_{\tilde{A}\tilde{b}}^{R}(I)\right)_{ij} = f_{\tilde{A}\tilde{b}}^{R}[r](x_{ij}),  \left(\tilde{f}_{\tilde{A}\tilde{b}}^{\tilde{E}}(F)\right)_{ij}^{Ab} = f_{\tilde{A}\tilde{b}}^{E}[e](x_{ij},A,b),\\
    &\forall i,j = 1,2,\cdots,n, \forall A,\tilde{A} \in S.
\end{split}
\end{equation}


\begin{theorem}
Assume that an image $I\in \mathbb{R}^{n\times n}$ is discretized from the smooth function $r:\mathbb{R}^2\to\mathbb{R}$ by (\ref{I}), a feature map $F\in \mathbb{R}^{n\times n \times t}$ is discretized from the smooth function $e:\mathbb{R}^2\times S\to\mathbb{R}$ by (\ref{F}), $|S|=t$, and filters $\tilde{\Psi}$, $\tilde{\Phi}$ and $\tilde{\Upsilon}$ are generated from $\varphi_{in}$, $\varphi_{out}$ and $\varphi_{A}, \forall A\in S$, by (\ref{Phi_d}), respectively. If for  any $A\in S,~ x\in \mathbb{R}^2$, the following conditions are satisfied:
\begin{align}\label{condition}
      &|r(x)| , |e(x,A,b)|\leq F_1,\\
            &\|\nabla r(x)\| , \|\nabla e(x,A,b) \|\leq G_1,\\
                  &\|\nabla^2 r(x) \| , \|\nabla^2 e(x,A,b) \|\leq H_1,\\
      &|\varphi_{in}(x)|, |\varphi_{A}(x)|, |\varphi_{out}(x)|\leq F_2, \\
       &\|\nabla \varphi_{in}(x) \|, \|\nabla \varphi_{A}(x) \|, \|\nabla \varphi_{out}(x) \|\leq G_2, \\
       &\|\nabla^2 \varphi_{in}(x)\|, \|\nabla^2 \varphi_{A}(x) \| , \|\nabla^2 \varphi_{out}(x) \|\leq H_2, \\
      &\forall \|x\|\geq\nicefrac{(p+1)h}{2},~ \varphi_{in}(x), \varphi_{A}(x), \varphi_{out}(x)  =0,
\end{align}

where $p$ is the filter size, $h$ is the mesh size, and $\nabla$ and ${\nabla}^2$ denote the operators of gradient and Hessian matrix, respectively, then for any $\tilde{A}\in S$, the following results are satisfied:
\begin{equation}\label{Thm3}
\begin{split}
   &\left\|\tilde{\Psi}\star\tilde{f}_{\tilde{A}\tilde{b}}^R\left(I\right) - \tilde{\pi}^{\tilde{E}}_{\tilde{A}}\left(\tilde{\Psi}\star I \right)\right\|_{\infty}
    \leq\frac{C}{2}(p+1)^2h^2  , \\
   &\left\|\tilde{\Phi}\star\tilde{f}_{\tilde{A}\tilde{b}}^{\tilde{E}}\left(F\right) - f_{\tilde{A}\tilde{b}}^{\tilde{E}}\left(\tilde{\Phi}\star F\right)\right\|_{\infty}
    \leq\frac{C}{2}(p+1)^2h^2t  ,\\
   &\left\|\tilde{\Upsilon}\star \tilde{f}_{\tilde{A}\tilde{b}}^{\tilde{E}}\left(F\right) - \tilde{f}_{\tilde{A}\tilde{b}}^R\left(\tilde{\Upsilon}\star F\right)\right\|_{\infty}
    \leq\frac{C}{2}(p+1)^2h^2t  ,
\end{split}
\end{equation}
where $C = F_1H_2+F_2H_1+2G_1G_2$, $\tilde{f}_{\tilde{A}\tilde{b}}^R$, $\tilde{f}_{\tilde{A}\tilde{b}}^{\tilde{E}}$, $\tilde{\Psi}$, $\tilde{\Phi}$ and $\tilde{\Upsilon}$
are defined by (\ref{Phi_d}) and (\ref{Pi_d}), respectively, the operators $\star$ involved in Eq. (\ref{Thm3}) are defined in (\ref{input_d}), (\ref{regular_d}) and (\ref{output_d}, respectively, and $\|\cdot\|_{\infty}$ represents the infinity norm.
\end{theorem} 
% \begin{proof}
% For the affine transformation, we have:
% \begin{equation}
%     f(x) = \pi_{\theta}x+b
% \end{equation}
% Then the inverse transformation of $f(\cdot)$ should be $f^{-1}(\cdot)=\pi_\theta^{-1}(x-b)$. In that, the left of Eq. \ref{eq:th1} can be rewritten as:
% \begin{align}
%  &~~~~~|f^{-1} \left[ g_{eq} \right] (f(X)) - g_{eq}(X) | \nonumber \\
%  & = \left|\pi_\theta^{-1}([g_{eq}](\pi_\theta X+b)-b)- g_{eq}(X)\right|\nonumber\\
%  &= \left|\pi_\theta^{-1}([g_{eq}](\pi_\theta X) + [g_{eq}](b)-b) -  g_{eq}(X)\right|\nonumber\\
%   &= \left|(\pi_\theta^{-1}[g_{eq}](\pi_\theta X) - g_{eq}(X)) + (\pi_\theta^{-1}([g_{eq}](b)-b)) \right|\nonumber\\
%   & \leq \left|(\pi_\theta^{-1}[g_{eq}](\pi_\theta X) - g_{eq}(X))\right| + |(\pi_\theta^{-1}([g_{eq}](b)-b))| \nonumber\\
%   & \leq |\pi_\theta^{-1}| (C (p + 1)^2 h^2) +  D
% \end{align}
% where $D = |(\pi_\theta^{-1}([g_{eq}](b)-b))| $ is positive constant.

% \end{proof}

\begin{theorem}
For an image $X$ with size $H \times W \times n_0$, and an $N$-layer rotation equivariant CNN network $G_{\text{eq}}(\cdot)$, whose channel number of the $i$th layer is $n_i$, rotation equivariant subgroup is $S \leq O(2)$, $|S| = t$, translation equivariant subgroup is $L \leq (\mathbb{R}^2, +)$, $|L| = l$, and the activation function is set as ReLU. If the latent continuous function of the $c$th channel of $X$ is denoted as $r_c: \mathbb{R}^2 \to \mathbb{R}$, and the latent continuous function of any convolution filters in the $i$th layer is denoted as $\phi_i: \mathbb{R}^2 \to \mathbb{R}$, where $i \in \{1, \cdots, N\}, c \in \{1, \cdots, n_0\}$, for any $x \in \mathbb{R}^2$, the following conditions are satisfied: 

\begin{align}
    |r_c(x)| \leq F_0, 
    \|\nabla r_c(x)\|\leq J_0, 
    \|\nabla^2 r_c(x)\|\leq H_0, \\
    |\phi_i(x)|\leq F_i, 
    \|\nabla \phi_i(x)\| \leq J_i, 
    \|\nabla^2 \phi_i(x)\| \leq H_i, \\
    \forall \|x\| \geq \frac{(p+1)h}{2}, \quad \phi_i(x) = 0.
\end{align}

where $p$ is the filter size, $h$ is the mesh size, and $\nabla$ and $\nabla^2$ denote the gradient and Hessian matrix operators, respectively. For an arbitrary $0 \leq \theta \leq 2\pi$, $A_\theta$ denotes the rotation matrix, $-N \leq p \leq N$, $b_p$ denotes the translation matrix and the following result is satisfied:
\begin{align}
| G_{\text{eq}}[f_{A_\theta b_p}](X) - f_{A_\theta b_p}[G_{\text{eq}}](X) | \leq C_1 h^2 + C_2 p h t^{-1},
\end{align}

\end{theorem}


\begin{theorem}
For an image $X$ with size $H \times W \times n_0$, and an $N$-layer rotation equivariant CNN network $G_{\text{eq}}(\cdot)$, whose channel number of the $i$th layer is $n_i$, rotation equivariant subgroup is $S \leq O(2)$, $|S| = t$, translation equivariant subgroup is $L \leq (\mathbb{R}^2, +)$, $|L| = l$, and the activation function is set as ReLU. If the latent continuous function of the $c$th channel of $X$ is denoted as $r_c: \mathbb{R}^2 \to \mathbb{R}$, and the latent continuous function of any convolution filters in the $i$th layer is denoted as $\phi_i: \mathbb{R}^2 \to \mathbb{R}$, where $i \in \{1, \cdots, N\}, c \in \{1, \cdots, n_0\}$, for any $x \in \mathbb{R}^2$, the following conditions are satisfied: 

\begin{align}
    |r_c(x)| \leq F_0, 
    \|\nabla r_c(x)\|\leq J_0, 
    \|\nabla^2 r_c(x)\|\leq H_0, \\
    |\phi_i(x)|\leq F_i, 
    \|\nabla \phi_i(x)\| \leq J_i, 
    \|\nabla^2 \phi_i(x)\| \leq H_i, \\
    \forall \|x\| \geq \frac{(p+1)h}{2}, \quad \phi_i(x) = 0.
\end{align}

where $p$ is the filter size, $h$ is the mesh size, and $\nabla$ and $\nabla^2$ denote the gradient and Hessian matrix operators, respectively. For an arbitrary $0 \leq \theta \leq 2\pi$, $A_\theta$ denotes the rotation matrix, $-N \leq p \leq N$, $b_p$ denotes the translation matrix and the following result is satisfied:
\begin{align}
&| f_{A_\theta b_p}^{-1}[G_{\text{eq}}](f_{A_\theta b_p}(X)) - G_{\text{eq}}(X) | \nonumber\\
& \leq max_{ij}|(G_{\text{eq}}[f_{A_\theta b_p}](X) - f_{A_\theta b_p}[G_{\text{eq}}](X) )_{ij}|,\\
&\leq C_1 h^2 + C_2 p h t^{-1},
\end{align}



\end{theorem}


\subsection{Our Method}


